Self-Explainable Graph Neural Networks for Link Prediction

Graph Neural Networks (GNNs) have achieved state-of-the-art performance for link prediction. However, GNNs suffer from poor interpretability, which limits their adoptions in critical scenarios that require knowing why certain links are predicted. Despite various methods proposed for the explainability of GNNs, most of them are post-hoc explainers developed for explaining node classification. Directly adopting existing post-hoc explainers for explaining link prediction is sub-optimal because: (i) post-hoc explainers usually adopt another strategy or model to explain a target model, which could misinterpret the target model; and (ii) GNN explainers for node classification identify crucial subgraphs around each node for the explanation; while for link prediction, one needs to explain the prediction for each pair of nodes based on graph structure and node attributes. Therefore, in this paper, we study a novel problem of self-explainable GNNs for link prediction, which can simultaneously give accurate predictions and explanations. Concretely, we propose a new framework and it can find various $K$ important neighbors of one node to learn pair-specific representations for links from this node to other nodes. These $K$ different neighbors represent important characteristics of the node and model various factors for links from it. Thus, $K$ neighbors can provide explanations for the existence of links. Experiments on both synthetic and real-world datasets verify the effectiveness of the proposed framework for link prediction and explanation.

==> introduction.tex <==
\section{Introduction}
\begin{figure}[t] 
\centering 
\includegraphics[width=0.5\textwidth]{illustration.pdf} 
\vskip -1.6em
\caption{Example of factors for the link between $v_i$ and $v_j$.} 
\label{illustration}
\vskip -1.6em
\end{figure}
% \suhang{come up with a better title, how about: self-explainable graph neural networks for link prediction}
Over the past few years, graph structured data is pervasive  in a wide spectrum of applications such as social networks~\cite{qu2021imgagn}, recommendation system~\cite{fan2019graph} and knowledge graphs~\cite{nickel2015review}. Since real-world graphs are often partially observed, link prediction, which aims to predict missing links, has been recognized as a fundamental task. For example, link prediction can be used to recommend new friends on social media~\cite{adamic2003friends}, predict protein interactions~\cite{qi2006evaluation} or reconstruct knowledge graphs~\cite{nickel2015review}. Existing link prediction methods can be generally split into two categories, i.e., heuristic-based approaches~\cite{lu2009similarity, newman2001clustering, adamic2003friends, katz1953new} and representation learning based approaches~\cite{acar2009link, kipf2016variational, zhang2018link, pan2022neural}. Early studies on link prediction compute some heuristic node similarity scores as the likelihood of links~\cite{lu2009similarity}. For example, common neighbors (CN) score a pair of nodes by the number of shared neighbors~\cite{newman2001clustering}. For representation learning based methods, Graph Neural Networks (GNNs) recently have achieved state-of-the art performance for link prediction~\cite{kipf2016variational, zhang2018link}. Generally, GNNs aggregate the neighbors' information to capture node attributes and local topology information to learn node embeddings and further facilitate the link prediction task.  

Despite the success in predicting missing links in graphs, predictions of GNNs are not interpretable for humans which limits their applications in various domains like recommendation systems, requiring the reason for predictions. GNNs are built upon a highly nonlinear entanglement of irregular graph features, making the predictions difficult to understand. To understand the inner working of the inference process of GNNs, various approaches have been studied to find significant patterns for the prediction by explaining GNNs~\cite{luo2020parameterized, ying2019gnnexplainer, schlichtkrull2020interpreting, yuan2020xgnn, yuan2021explainability}. For instance, GNNExplainer~\cite{ying2019gnnexplainer} provides crucial node attributes and subgraphs which affect the predictions most from a trained GNN model. The model-level explanation is also studied to generate graph patterns for a target class~\cite{yuan2020xgnn}. However,  all the aforementioned models  focus on the post-hoc explanations, i.e., learning an additional explainer for a trained GNN model. Since the learned explanations in post-hoc ways are not directly obtained from GNNs, they can misrepresent the true explanations of the GNNs~\cite{rudin2019stop}. There are very few initial efforts for self-explainable GNNs~\cite{dai2021towards, zhang2022protgnn}. Also, previous self-explainable models are designed to find explanations for node or graph classification. Nevertheless, explanations of links between nodes may require unique patterns and it's hard to apply them to link prediction directly. Therefore,  it is crucial to develop a self-explainable GNN for link prediction, which can simultaneously give predictions and explanations.

In real-life graphs, links from one node to other nodes may result from different factors. For example, as shown in Figure~\ref{illustration}, in the social networks, the node $v_i$ has broad interests in football, arts and music. Therefore, it builds links with different users based on common interests between them. The missing link of $(v_i, v_j)$ may be from their interests in music. It's hard to predict the link based on their feature of interest because most of their interests are different. Therefore, we should learn pair-specific representations of them, which preserve their common interest in music and represent factors of the link. Generally, the interests of users are reflected in their neighbors. In this case, the most similar neighbors of $v_i$ to $v_j$ denote interests in music, which is the factor of the link. Similarly, the most similar neighbors of $v_j$ are also interested in music. Thus, by aggregating these neighbors, we can predict the link correctly. Based on this case, for each node pair $(v_i, v_c)$, one way to obtain self-explainable link prediction is to find dominating $K$ neighbors of $v_i$, which represent the factors of building links of $(v_i, v_c)$, sharing top $K$ similarity with $v_c$.  Specifically, the explanation for whether there is a link for $(v_i, v_c)$ can be: \textit{(i)} ``A link predicted for $(v_i, v_c)$ is because $K$ neighbors of $v_i$ represent common feature with $v_c$. And common feature shared for node pairs is the factor of the link between $v_i$ and $v_j$ and \textit{(ii)} ``no link predicted for $(v_i, v_c)$ is because even top $K$ similar neighbors of $v_i$ w.r.t $v_c$ don't share common feature with $v_c$, which represent no potential factor of the link''. This explanation also holds true for the node $v_j$. Though promising, the work on exploring $K$ relevant neighbors for self-explainable GNNs on link prediction is rather limited.

Therefore, in this paper, for each node pair $(v_i, v_j)$, we investigate a novel problem of self-explainable GNN for link prediction by exploring $K$ important neighbors of $v_i$ which are similar to $v_j$. Similarly, this  self-explainable GNN should also explicitly identifies $K$ important neighbors of $v_j$ which are similar to node $v_i$. However, this is a non-trivial task. There are two main challenges: (\textit{i}) how to incorporate the node similarity and
high-order structure similarity to identify $K$ important neighbors? One straightforward solution is using the cosine similarity of node representations learned by GNNs~\cite{kipf2016semi, velivckovic2017graph}. However, most of GNNs are two-layer neural networks which only capture local structure and node attribute information. Deeper GNNs modeling high-order neighbors information will learn poor representation due to over-smoothing issues~\cite{li2018deeper,alon2020bottleneck}, and are also time-consuming. Since original local topology structures are often sparse and missed in real-world graphs, it's necessary to use an efficient method to explore high-order structure information; and (\textit{ii}) how to give both accurate predictions and correct corresponding explanations? The supervision we have is only from the information on observed links. How to use them to enhance explanations is required to be investigated. 

In an attempt to solve the challenges, we propose a model named Interpretable Link Prediction based on Graph Neural Networks (ILP-GNN). For each node pair $(v_i, v_j)$, ILP-GNN adopts a novel mechanism that can explicitly evaluate the node similarity and high-order structure similarity to find $K$ interpretable neighbors of $v_i$ similar to $v_j$, where these neighbors can represent common interest or feature between $v_i$ and $v_j$. For high-order structure similarity, graph diffusion is utilized to calculate the closeness of nodes by modeling their local and high-order neighbors' information~\cite{klicpera2019diffusion}. Then, these $K$ neighbors are aggregated to learn pair-specific representation, which represents common features of node pairs and various factors of links for different node pairs. Furthermore, since explanation based on selecting $K$ important neighbors should preserve factors resulting in the existence of links, we propose a novel loss function to encourage explanation of our model and improve the performance of link prediction. The main contributions are:
\begin{itemize}[leftmargin=*]
\item We study a novel problem of self-explainable GNN for link prediction by finding $K$ neighbors which are relevant to the links. 
\item We develop a novel framework ILP-GNN, which adopts an interpretable neighbors aggregation method to identify $K$ relevant neighbors to factors leading to links and enhance the explanations with a novel loss function;
\item We construct a synthetic dataset which can quantitatively evaluate the link prediction explanation.
\item We conduct extensive experiments on both real-world and synthetic datasets to demonstrate the effectiveness of our model to give accurate predictions and explanations.
\end{itemize}




% \suhang{Huaisheng, after reading your problem definition and part of methdology, I think the motivation of selecting $K$ neighbors is not clearly explained. The intuition should be something like this (just rough idea, you need to rephrase the sentences): Generally, nodes are linked due to various factors. For example,in social networks, user $v_i$ and user $v_j$ are connected because they share common interest in sports; while $v_i$ and $v_k$ are connected might because they are both interested in music. In other words, for the same node $v_i$, we need different representations of $v_i$ when we want to predict the link of $v_i$ with different nodes. To predict link between $v_i$ and $v_j$, we need to learn representations of $v_i$ and $v_j$ that can capture common interests between them; while to predict the link between  $(v_i$ and $v_k$, we need to learn another representation of $v_i$ that preserve similarity with  $v_k$. Simply apply GNN that aggregate the neighborhood of $v_i$ to learn one representation would be helpful for node classification, but sub-optimal for link prediction. However, for a pair of node $(v_i,v_j)$, how can we mine the similarity between them remains a question. pair-specific representation}

% \suhang{Generally, the characteristics/preferences of a node is reflected in his neighborhood. This is where you will talk about why we would compare similarity of $v_j$ with neighborhood of $v_i$. Explain the intuition. For $(v_i,v_j)$, not all neighbors are important for their link prediction because each of them can have diverse interests. xxxx.}
